Introduction to Neural Network Verification

Deep learning has transformed the way we think of software and what it can do. But deep neural networks are fragile and their behaviors are often surprising. In many settings, we need to provide formal guarantees on the safety, security, correctness, or robustness of neural networks. This book covers foundational ideas from formal verification and their adaptation to reasoning about neural networks and deep learning.

==> bibliography.tex <==
\bibliographystyle{plainnat}
\addcontentsline{toc}{chapter}{\hlvr References}
\bibliography{fnt/refs}

==> fnt/FnTarticle-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {FnTarticle}


==> fnt/FnTarticle-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {FnTarticle}


==> fnt/FnTarticle-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {FnTarticle}


==> fnt/FnTarticle-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {FnTarticle}


==> fnt/FnTarticle-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {FnTarticle}


==> fnt/FnTarticle-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {FnTarticle}


==> fnt/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> fnt/absintdl.tex <==
\chapter{Abstract Deep Learning}\label{ch:absintdl}

==> fnt/main-nowbook.tex <==
\PassOptionsToClass {book,biber}{nowfnt}
\input {main}


==> fnt/main-nowchapter.tex <==
\PassOptionsToClass {chapter,biber}{nowfnt}
\input {main}


==> fnt/main-nowebook.tex <==
\PassOptionsToClass {ebook,biber}{nowfnt}
\input {main}


==> fnt/main-nowechapter.tex <==
\PassOptionsToClass {echapter,biber}{nowfnt}
\input {main}


==> fnt/main-nowplain.tex <==
\PassOptionsToClass {plain,biber}{nowfnt}
\input {main}


==> fnt/main-nowsample.tex <==
\PassOptionsToClass {sample,biber}{nowfnt}
\input {main}


==> fnt/preamble.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PACKAGES
%
%don't mess with physics
\newcommand\hmmax{0}
\newcommand\bmmax{0}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{hyperref} % no colorful hyperlinks
% \usepackage{mathpazo} % math & rm
% \usepackage[T1]{fontenc}
\usepackage{titlesec} % modify sec/subsec/etc.
\usepackage{epigraph}
\usepackage{blindtext} % temporary
\usepackage[dvipsnames]{xcolor}
\usepackage{tikz}
\usepackage{dsfont}
\usepackage{pgfplots}
\usepackage{float}
\usepackage[capitalize,noabbrev]{cleveref}
\usepackage{bm}
\usepackage{csquotes}
\usepackage{stmaryrd}
\usepackage{wasysym}
\usepackage{mathtools}
\usepackage{paralist}
\usepackage{enumitem}
\usepackage[ruled,noend]{algorithm2e}
\usepackage{listings}
\usepackage[defaultsans,scale=0.95]{opensans} 
\hypersetup{
  linkcolor  = Black,
  citecolor  = RoyalBlue,
  urlcolor   = RoyalBlue,
  colorlinks = true,
}

% \usepackage{arabtex}
% \renewenvironment{abstract}%
%          {\centerline{\large\bf Abstract}%
%           \begin{list}{}%
%              {\setlength{\rightmargin}{0.6cm}%
%               \setlength{\leftmargin}{0.6cm}}%
%            \item[]\ignorespaces}%
%          {\unskip\end{list}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math and symbols


% \newcounter{example}[chapter]

% \renewtheorem{example}{Example}[section]


% \renewenvironment{example}[1][]{\vspace{1em}\refstepcounter{example}\par\medskip
% \noindent {\small{\sfseries { Example}~{\theexample}  #1}} \rmfamily}{\hfill\scriptsize\ensuremath{\blacksquare}\medskip\vspace{1em}}

% \renewcommand*{\theexample}{\thechapter.\Alph{example}}

% \makeatletter  
% \def\@endtheorem{$\blacksquare$\endtrivlist\@endpefalse } % insert `\qed` macro
% \makeatother

% \newcounter{theorem}[chapter]

% \newenvironment{theorem}[1][]{\refstepcounter{theorem}\par\medskip
% \noindent {\small{{\hlv Theorem}~{\hlvr\thetheorem}  #1}} \rmfamily}
% {\hfill\scriptsize\ensuremath{\blacksquare}\medskip}

% \renewcommand*{\thetheorem}{\thechapter.\Alph{theorem}}

% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}

\renewcommand{\vec}[1]{\bm{#1}}
\renewcommand{\geq}{\geqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\iff}{\Leftrightarrow}

\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % Fonts and margins

% % same margins on even/odd
% \setlrmargins{*}{*}{1}
% \checkandfixthelayout

% % import Open Sans TODO: change names to something meaningful
% \newfontfamily{\hlv}[UprightFont={* Bold}] {Open Sans}
% \newfontfamily{\hlvm}[UprightFont={* SemiBold}] {Open Sans}
% \newfontfamily{\hlvr}{Open Sans}
% \newfontfamily{\hlvl}[UprightFont={* Italic}]{Open Sans}

% \newfontfamily{\tfontb}[ UprightFont={* Bold}] {Open Sans}
% \newfontfamily{\tfontr}{Open Sans}


% \linespread{1.1}        % Palatino needs more leading (space between lines)

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % TABLE OF CONTENTS
% %

% % TOC Title font
% \renewcommand\printtoctitle[1]{\Large\hlv Table of Contents}

% % TOC Chapter and section fonts
% \renewcommand\cftchapteraftersnumb{\footnotesize\normalfont\hlvr}
% \renewcommand\cftchapterpresnum{\footnotesize\normalfont\hlvr}

% \renewcommand\cftsectionaftersnumb{\footnotesize\hlvl}
% \renewcommand\cftsectionpresnum{\footnotesize\hlvl}

% \renewcommand\cftbeforechapterskip{2pt plus 1pt}
% \renewcommand\cftbeforepartskip{20pt plus 1pt}

% % TOC Part font
% \renewcommand\cftpartaftersnumb{\small\hlvr}
% \renewcommand\cftpartpresnum{\small\hlvr}
% \cftpagenumbersoff{part} % no page number on parts


% % TOC page number format
% \renewcommand*{\cftchapterformatpnum}[1]{~~{\footnotesize\hlvl #1}}
% \renewcommand*{\cftsectionformatpnum}[1]{~~{\footnotesize\hlvl #1}}
% \renewcommand*{\cftsubsectionformatpnum}[1]{~~{\hlvl #1}}

% % TOC Page numbers next to chapter/section instead of right aligned
% \renewcommand*{\cftchapterleader}{}
% \renewcommand*{\cftsectionleader}{}
% \renewcommand*{\cftsubsectionleader}{}

% % TOC don't spread entry across line -- left align
% \renewcommand{\cftchapterafterpnum}{\cftparfillskip}
% \renewcommand{\cftsectionafterpnum}{\cftparfillskip}
% \renewcommand{\cftsubsectionafterpnum}{\cftparfillskip}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Headers/footers
% %

% \makepagestyle{headings}

% \makeatletter      
% % headers
% \makeevenhead{headings}{\footnotesize\hlvr\thepage}{}{\footnotesize\hlvr\MakeUppercase{\leftmark}}
% \makeoddhead{headings}{\footnotesize\hlvr\MakeUppercase{\rightmark}}{}{\footnotesize\hlvr\thepage}

% % no footers
% \makeoddfoot{headings}{}{}{\hlvr \tiny \MakeUppercase\today}
% \makeevenfoot{headings}{\hlvr \tiny \MakeUppercase\today}{}{}
% \makeatother

% \makepagestyle{chapterstyle}

% \makeatletter      
% % headers
% \makeevenhead{chapterstyle}{}{}{}
% \makeoddhead{chapterstyle}{}{}{\footnotesize\hlvr\thepage}

% % no footers
% \makeoddfoot{chapterstyle}{}{}{\hlvr \tiny \MakeUppercase\today}
% \makeevenfoot{chapterstyle}{\hlvr \tiny \MakeUppercase\today}{}{}
% \makeatother   %

% % page style for chapters, parts, toc
% \aliaspagestyle{chapter}{chapterstyle}
% \aliaspagestyle{part}{empty} % nothing in part page
% \aliaspagestyle{cft}{headings}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Part, chapter, paragraph, section formats + CAPTIONS
% %

% %chapter
% \titleformat{\chapter}[display]
% {\hlv\huge}
% {\hlvr\Large\chaptertitlename~\thechapter}
% {0ex}
% {
% }
% [\vspace{0ex}]


% % Part font
% \renewcommand*{\partnumfont}{\hlvr\huge}
% \renewcommand{\partnamefont}{\hlvr\huge\flushleft}
% \renewcommand{\parttitlefont}{\hlv\huge\flushleft}


% % Part spacing
% \renewcommand{\midpartskip}{}
% \renewcommand{\beforepartskip}{}
% \renewcommand{\afterpartskip}{}


% % section
% \titleformat{\section}[hang]{}{\large\hlvr\thesection}{0.5em}{\large\hlvr\bfseries}

% %subsection
% \titleformat{\subsection}[hang]{}{}{0pt}{\hlv}

% % subsection and section spacing
% \titlespacing*{\section}
% {0pt}{5.5ex plus 1ex minus .2ex}{2.3ex plus .2ex}
% \titlespacing*{\subsection}
% {0pt}{5.5ex plus 1ex minus .2ex}{1.5ex plus .2ex}

% %paragraph
% \let\originalparagraph\paragraph
% \makeatletter
% \renewcommand\paragraph{%%
%   \@startsection{paragraph}%%                        name                
%                 {4}%%                                level               
%                 {\z@}%%                              indentation         
%                 {2ex \@plus1ex \@minus.2ex}%%        beforeskip
%                 {-1em}%%                             afterskip
%                 {\hlvr\small\bfseries}}%% style
% \makeatother

% % captions
% \captionnamefont{\small\hlv}
% \captiontitlefont{\small\hlvr}
% \captiondelim{\hspace{0.5em}}
% % \captionstyle[\raggedright]{}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Quotes 
% \epigraphfontsize{\small}
\setlength\epigraphwidth{9cm}
\setlength\epigraphrule{0pt}

% Footnotes

% no number footnote
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Custom title page
% %
% \title{Verified Deep Learning}
% \author{\hlvr Aws Albarghouthi}

% \newcommand*{\titleTH}{\begingroup% T&H Typography
% \noindent
% {\large \tfontb VERIFIED DEEP LEARNING}\\
% {\tfontr AWS ALBARGHOUTHI}\\[0.167\textheight]
% {\footnotesize\color{red}\MakeUppercase{\tfontr In progress; do not circulate}}\\
% {\footnotesize\MakeUppercase {\tfontr Last updated: \today}}\\[0.167\textheight]
% \endgroup}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Tikz stuff

%config
\usetikzlibrary{arrows,backgrounds,decorations.markings}
\usepgflibrary{shapes.multipart}
\usetikzlibrary{patterns,calc}

\makeatletter
\newcommand{\pgfplotsdrawaxis}{\pgfplots@draw@axis}
\makeatother

\pgfplotsset{only axis on top/.style={axis on top=false, after end axis/.code={
             \pgfplotsset{axis line style=opaque, ticklabel style=opaque, tick style={thick,opaque},
                          grid=none}\pgfplotsdrawaxis}}}

\tikzset{>=latex} % arrows

% nodes
\tikzstyle{oper}=[circle, draw=black, thick, minimum size = 8mm]
\tikzstyle{input}=[rounded corners, draw=Maroon, thick, minimum size = 6mm]
\tikzstyle{output}=[rounded corners, thick, draw=RoyalBlue, minimum size = 6mm]
\tikzstyle{empty}=[circle, draw=white, opacity=0, minimum size = 1mm]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% lists

\setlist[description]{
    labelindent=.5cm,
    style=unboxed,
    leftmargin=.5cm,
    %font=\small\hlvr,
%    topsep=3pt,
%    itemsep=-.5ex
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% algorithms -- algorithm2e
\Crefname{algocf}{Algorithm}{Algorithms} %algorithms not natively supported
\newcommand{\acomment}[1]{ {\color{Blue} $\triangleright$ #1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% code
\lstdefinestyle{customc}{
  belowcaptionskip=1\baselineskip,
  breaklines=true,
  xleftmargin=\parindent,
  language=C,
  showstringspaces=false,
  basicstyle=\ttfamily,
  keywordstyle=\bfseries\ttfamily\color{MidnightBlue},
  commentstyle=\itshape\color{black},
  identifierstyle=\ttfamily\color{black},
  stringstyle=\itshape\color{blue},
  keywords={ map,  while, flatMap, reduce, then, in, return,  for, if, else, reduceByKey, filter, partition},
  % attributestyle = \ttfamily\color{Mahogany}
}

\lstset{columns=fullflexible,
        mathescape=true,
        literate=,
        basicstyle=\ttfamily,
        numbersep=5pt,
        numberstyle=\tt\color{gray}
}
\lstset{escapechar=@,style=customc}

%space above and below
\lstset{aboveskip=4pt,belowskip=4pt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{macros}


==> titlepage.tex <==
\begin{titlingpage}
\titleTH
\end{titlingpage}




==> toc.tex <==
\tableofcontents*

